Merge: An Architecture for Interconnected Testbed Ecosystems

In the cybersecurity research community, there is no one-size-fits-all solution for merging large numbers of heterogeneous resources and experimentation capabilities from disparate specialized testbeds into integrated experiments. The current landscape for cyber-experimentation is diverse, encompassing many fields including critical infrastructure, enterprise IT, cyber-physical systems, cellular networks, automotive platforms, IoT and industrial control systems. Existing federated testbeds are constricted in design to predefined domains of applicability, lacking the systematic ability to integrate the burgeoning number of heterogeneous devices or tools that enable their effective use for experimentation. We have developed the Merge architecture to dynamically integrate disparate testbeds in a logically centralized way that allows researchers to effectively discover, and use the resources and capabilities provided the by evolving ecosystem of distributed testbeds for the development of rigorous and high-fidelity cybersecurity experiments.

==> abstract.tex <==
%!TEX root = ceftb.tex
\subsection*{Abstract}
In the cybersecurity research community, there is no one-size-fits-all solution for \emph{merging} large numbers of heterogeneous resources and experimentation capabilities from disparate specialized testbeds into integrated experiments. The current landscape for cyber-experimentation is diverse, encompassing many fields including critical infrastructure, enterprise IT, cyber-physical systems, cellular networks, automotive platforms, IoT and industrial control systems. Existing federated testbeds are constricted in design to predefined domains of applicability, lacking the systematic ability to integrate the burgeoning number of heterogeneous devices or tools that enable their effective use for experimentation. We have developed the Merge architecture to dynamically integrate disparate testbeds in a logically centralized way that allows researchers to effectively discover, and use the resources and capabilities provided the by evolving ecosystem of distributed testbeds for the development of rigorous and high-fidelity cybersecurity experiments.
%not presuppose the domain of experimentation or set of resources provided by any testbed. 

%(i) is agnostic to resource complexity and is able to evolve with new technologies, 
%(ii) separates realization (mapping resources) and materialization (implementing the mapping) to provide experimenters with interactive and iterative experiment design, 
%(iii) provides a novel method of describing resources and experiments, 
%(iiii) gives resource providers proactive control 

%LT: points {i} and {iii} are very similar, and especially since we have essentially eliminated experiment design, this point is weak.
%We propose the \M architecture for assimilating heterogeneous devices, across testbeds into a common ecosystem that can be leveraged to \emph{express}, \emph{realize} and \emph{materialize} cyber-experiments. 
% SR: the above sentence seems too generic
%Conceptually, the \M architecture makes the following contributions: (i) an open ended \emph{experiment representation}, (ii) a \emph{constraint based realization engine} and (iii) a \emph{distributed materialization runtime} based around the operating system driver model.
%Presently there is no integration framework that can provide for diverse experimentation addressing the following problem space:
%(i) how are experiments \emph{expressed}, (ii) how are they \emph{realized} and (iii) how does the underlying testbed infrastructure \emph{evolve} to accommodate new types of (physical or virtual) resources with minimal overhead for the resource provider and experimenter.


==> exp.tex <==
\section{\M: Experimenter API}
\label{exp}
\todo[inline]{Rewrite again, to be more of a cohesive story with fewer details. Will need some rework still. Are we capturing the right main points? --gen.}
In Merge, creating an experiment is an iterative process. 
During this process, the user describes 
 their experiment's structural requirements, such as topology 
 and hardware specifications
 and the behavior required of these resources---i.e. how these resources will   interact.
The system uses resource discovery to evaluate if the specified requirements can be  met, and if not, the design process iterates. 
A user may over- or under-specify her experiment requirements.
If the experimenter over-specifies requirements, 
 there will be no realizable experiment configuration,
  and the API must work with the user to iteratively 
  1) discover what resources are available and 2) help the user relax her  constraints.
 In the case under-specification, 
   the API must interactively work with the user to identify more requirements
   and/or offer realizable configurations. 

For the Merge architecture, we created Common Open Model Expression Toolkit (Comet), which is able to describe an experiment's structural and behavior requirements as shown in Figure~\ref{Comet}. 
Comet is able to describe both topology, 
 like NS2/3~\cite{ns},
 and behavior, 
 like OMF~\cite{omf} or MAGI~\cite{magi}.
 
Comet is not the only pathway to describing experiments. 
Contributors can write their own toolkit or UI to interface with the experimenter API to produce, at the very minimum, a description of the experiment's structural realization in XIR.

Comet captures graphs of entities and constraints about these graphs. 
Topology can easily be understood as a graph structure, where nodes in the graph represent entities, and arcs represent how these entities are connected. 
Behavior can also be represented as a graph. 
In Comet, the nodes in a behavior graph  represents events. 
Event nodes are connected by arcs representing triggers between events. 

%For example, if an experimenter wants to start an attack script which attempts to overload a web server, but only after the web server has been set up and started, the Comet graph to represent this desired behavior would have two event nodes, a ``web server start'' and ``attack start'', connected by a arc representing the successful start of the web server.

%Comet produces a structure which is realizable, but also captures the environment and behavior of resources through our eXperiment Development Containers (XDC). 
%Anything that the experiment requires in terms of data, device configurations, software etc. can be included in the container itself, thus reducing the burden of setting up resources, and promoting sharing and reusability.

%We've also built a specialized XDC container that includes a Jupyter~\cite{jupyter} instance.  
%Jupyter enable users to interactively run and modify code in a rich web-based shell environment that supports graphics. Our Comet %Python bindings have functionality that is Jupyter aware, allowing users to interact with the structural and behavioral aspects of their experiments using Jupyter widgets.
%This way when a user wants to interact with their experiment container, they can just fire up the container, point their web browser at the containers IP address and use Jupyter to interact with their experiment.


%\todo[inline]{Below is the old text. Above is suggested text.}
%To improve on the ability for experimenters to have repeatable and verifiable experiments, we have created eXperiment Development Containers (XDC). They act much like normal containers, with each layer being a composition of the previous layers and the current modifications. In the same way, we are able to describe experiments as a composition of layers that include the data, programs, structural and behavioral specifications, and any other elements that may comprise an experiment. Running a normal container typically executes a program that provides a service. Running an XDC container, executes a structural or behavioral comet model that results in an experiment package that can be shared or sent to the core for realization and materialization. Because this is a containerized setting, anything that the model experiment model requires in terms of data, device configurations, software etc. can be included in the container itself. 

%\todo[inline]{\textbf{Alefiya, Gen, Jelena}}
%\todo[inline]{We should make the point that we're modular enough to easily support multiple UIs (as long as the UI can spit out Comet, we don't care what the UI is, right?) and then we can talk about using Jupityer Notebooks. Not sure where this point goes as this section is about the experience of using things top to bottom (I'm guessing we should say something earlier than here.) --Gen}

%We've also built a specialized XDC container that includes a Jupyter \cite{jupyter} instance.  Jupyter enable users to interactively run and modify code in a rich web-based shell environment that supports graphics and pretty much any other type of media supported by web browsers. Our Comet Python bindings have functionality that is Jupyter aware, allowing users to interact with the structural and behavioral aspects of their experiments using Jupyter widgets. This way when a user wants to interact with their experiment container, they can just fire up the container, point their web browser at the containers IP address and use Jupyter to interact with their experiment.

%RY[snip]: There are many problems with the below. Jupyter is like bash on crack with graphics, its not an implementation of an interface to Merge. One can interface with Merge from jupyter because jupyter can execute code and we have code that interacts the Merge's actual interface which is specified via OpenAPI. There is also conflation here with regard to the merge experimentation interface and experiment representation.
%---------
%Within a Jupyter notebook, users can describe the entirety of their experiment. The goal is to make sharing experiments easier within the experimental community by providing an environment where an experiment in its entirety can be wrapped up in an artifact that can be directly shared.  Jupityer Notebooks is the implementation of our interface to Merge, but by its very nature, any interface can be used, if for example an experimenter would prefer to keep their experiments in RSpec \cite{rspec}, that is also doable.
%---------

%\todo[inline]{need reality check on the interface between Model/Design and Explore, last sentence of paragraph - LT}

%Modeling is the first stage in creating a Merge experiment. This is where the experiment is designed - from what resources are needed, to how the resources are programmed to interact with each other.  There are some languages which can define the structural requirements from a testbed \cite{ns}, while others allow users to specify the behavior conditions of their experiment \cite{omf,magi}.  For the Merge architecture, we created Common Open Model Expression Toolkit (Comet), which is able to describe an experiments structural and behavior requirements as shown in Figure \ref{Comet}.  As mentioned before, it is not necessary that an experimenter use Comet, all that is required by modeling phase is that a graph representation can be passed to the Explore stage. 

%\todo[inline]{Rewrote this to make behavior less of a random add-on.  --Gen}
%Comet captures graphs of entities and constraints about these graphs. Topology can easily be understood as a graph structure, where nodes in the graph represent entities, and arcs represent how these entities are connected. Behavior can also be represented as a graph. In Comet, the nodes in a behavior graph  represents events. Event nodes are connected by arcs representing triggers between events. For example, if an experimenter wants to start an attack script which attempts to overload a web server, but only after the web server has been set up and started, the Comet graph to represent this desired behavior would have two event nodes, a ``web server start'' and ``attack start'', connected by a arc representing the successful start of the web server.
 
%To express constraints Comet implements standard operators such as $<$, $>$, $<=$, $>=$, $=$, as well keywords \textit{select} and \textit{choice}. For topology descriptions, this allows experimenters express constraints such as ``I would like a node with an x86 processor, and at least two physical cores''.  
% The below seems too detailed to include.
%In Comet, this statement translates to: \{`hardware': \{`arch=': `x86', `cpu$>$': `2'\} \}.  
%The standard mathematical operators are straightforward for allowing experimenters to define and relax constraints.  The keyword \textit{choice} is used for specifying a resource ordering, for example specifying that the experiment would prefer modern Intel processors (Skylake $>$ Haswell $>$ Sandy Bridge). Using the \textit{select} keyword each variable would be equally likely. For behavior descriptions, these operators allow the user to describe what entities carry out each event. For example, if a user wants to run an event on at least three machines, she could specify this with $>=$.

%Comet also allows for \textit{composition}, allowing variables to be defined at compile time.  
%This feature is useful for using environment variables or automation to define a set of constraints.  

%RY:[snip]
\begin{comment}
\begin{figure}[htp]
    \centering
    \includegraphics[width=.4\textwidth, height=.6\textheight]{img/jupiter-placeholder.png}
    \caption{Placeholder for jupityer/COMET}
    \label{Comet}
\end{figure}
\end{comment}

%\subsection{Experiment Structure}
%\subsection{Experiment Behavior}
%\subsection{Resource Composition}
%\subsection{Resource Capability}


==> system-new.tex <==
% RY: move the state machine specifics into the system design bits - not appropriate for architecture overview
%\section{System Design}
%
\section{Core Components}
\label{core}
%The purpose of the core components are to manage experiments, resources, and a set of runtime objects that bring the two together in a system that is useful for experimentation. 
%The primary runtime objects are \emph{realization mappings} and \emph{materialization stateboards}. A realization mapping maps experiment elements on to resource elements and act primarily as an allocation mechanism.
%A materialize stateboard is a state model that keeps track of what state a resource is currently in and what state it is supposed to be in. 
%This state model is borrowed from the Kubernetes \cite{kube} design.
%All state is kept within the core, which is logically centralized. 
%The reasoning behind this will become clear when we discuss algorithms in the realization section. 
% LT: reasoning isnt clear - it is also repeated in materialization section

\begin{comment}
%RY: This is not a list of core service, ceph for example is an implementation detail, what is important in that regard is an active-active CDN that sites can lean on for reliable distributed storage with reasonable performance.
\begin{itemize}
\item Ceph Cluster
\item Commander Commissioner
\item eXperimental Development Containers
\item Explore, Realize, Gather API
\end{itemize}
\end{comment}

In this section we describe the services that make up the Merge core. 
%The core services are designed to be microservices. 
The core services partition the Merge's functionality into four independent subsystems that communicate with each other through well defined \texttt{protobuf} \cite{protobuf} interfaces.
%Name resolution is assumed between each of the core services.
Each of the core services is stateless.
This makes replication and subsequently fault-tolerance schemes that are based on a replication model easy to implement from a system design point of view.
The services gather their required state from a set of databases. 
The only thing that is required of the databases, is that they support transactions. 
This is necessary because both the realization and materialization services employ optimistic concurrency techniques and require transactions to maintain correctness.
As we describe each of the core services, the modeling representation XIR, as it specifically pertains to each service will be presented in context.
%It is also necessary we distinguish between data that is durable vs data that is transient.
%For example an experiment is a durable piece of data and it evolves relatively slowly as the experimenter develops the experiment.
%A realization or materialization is transient and evolves relatively quickly as the realization and materialization engines work to compute the associate realization-mappings and materialization state-tables.
% LT: Last 3 sentences go somewhere else, they dont fit in this paragraph or section.

%\todo[inline]{LT: we need an XIR discussion before we talk about the services - what does it mean to model.  Has not be approached yet}

%To show the flexibility of the architecture, we have put together two reference system designs. The basic reference design simply deploys the core services and databases as a set of singleton containers interconnected by a common network. This environment is easy to deploy, is lightweight in terms of required resources and is ideal for rapid development. A simple \texttt{docker-compose up} can have the entire portal model up in under a minute. However, this system design is not appropriate for production. If a single service fails the whole system is crippled, and if a database is lost, tragedy ensues.

%The production reference system design is a triply redundant system e.g., each service and each database is has three replicas. There are also load balancing mechanisms that provide for performance and a level of fault tolerance. This system design uses Kubernetes to deploy and orchestrate the core services. The database redundancy is a function of the chosen technology. In both reference designs we employ an SQL type database for durable data and key-value type databases for transient data. In the production design Galera clustering is used for durable replication and Etcd clustering is used for transient replication. This reference design is depicted in Figure~\ref{portal}.

%\begin{figure}[ht]
%    \centering
%    \includegraphics[width=.95\columnwidth]{img/portal}
%    \caption{Production Reference Design}
%    \label{portal}
%\end{figure}

%RY: TODO fit the CDN storage model aspect more cleanly into the narrative, noting that the fact that it is Ceph based does not matter from an arch standpoint, we certainly should mention that Ceph provides a production quality CDN active-active replication solution that we can use, but the focus is we are creating a CDN capability for the sites.
\begin{comment}
For experimenters who require storage that either exists in another testbed, or are necessary to store output of an experiment, we use an active-active Ceph cluster\cite{ceph}.  The kernel uses the storage medium to store experiment meta data, while the experiment uses the cluster for permanent storage that is able to survive beyond the lifetime of the experiment.
\end{comment}

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%         Discovery & Realization
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Discovery \& Realization}
\label{discover}
\label{realize}

% \todo[inline]{\textbfI{Jim} - Alefiya made a good point, is it possible to get some evaluation from how long it takes to do SAT solving on what may be a realistic experiment parameters}

%One problem in the testbed community that we alluded to earlier is the virtual network embedding problem \cite{vni,emulab} which states that the mapping of a virtual topology onto a physical topology is NP-hard.
%In Merge parlance we call this process \emph{realization}, as it is selecting the resources with which to make an experiment \emph{real}. 

%RY[snip]: We will cover this a little more in-depth in the next section, however part of our success with limiting the amount of time to map resources is by creating a framework where the complexity and heterogeneity of devices is captured by XIR;  making the APIs simple, representing an infinite device space, and allowing very quick realizations.
%LT: my issue with this section is that it goes nowhere, rather that mention it and talk about it later, the two should be the same, where it is first mentioned - it is discussed, otherwise the reader is keeping track of too much state.

%A problem that is very much related to realization is \emph{discovery}.
%With realization, an experimenter submits a model of an experiment and Merge will come back with the lightest weight possible realization of that experiment that it can compute.
%Discovery is the second step of the experiment life cycle for an experimenter.
%An experimenter, models their experiment, and needs to find the necessary resources to implement their experiment.
The \textbf{discovery} process computes a map of an experiment network $\bm{x}$ onto a candidate map $\bm{c}$.
\begin{equation}
  \bm{x} := (\bm{n}_x, \bm{l}_x) \mapsto \textbf{c}(t) := (\bm{n}_x, \bm{N}_r(t))
\end{equation}
Here the $\bm{n}_x$ are experiment nodes, $\bm{l}_x$ are experiment links and $\bm{N}_r$ is a superset of resource nodes. When taken together $(\bm{n}_x, \bm{N}_r)$ is a map from each experiment node $n \in \bm{n}_x$ to a set of satisfying resource nodes $N \in \bm{N}_r$.

This mapping lets the experimenter see what is out there in terms of useful resources for their experiment. The process is depicted graphically in Figure ~\ref{disco}. 

%Discovery is a simple process of using XIR's tags to find relevant resources.
%Realization and discovery are depicted graphically in Figure~\ref{discoreal}.

%RY: yes I know - this diagram is not legible - later.....
\begin{figure}[ht]
    \centering
    \includegraphics[width=.95\columnwidth]{img/disco}
    \caption{Discovery of resources for an experiment}
    \label{disco}
\end{figure}

The \textbf{realization} process is very similar to the discovery process. However, instead of mapping an experiment network onto a candidate map, it is mapped onto a resource network $\bm{r}$.
\begin{equation}
  \bm{x} := (\bm{n}_x, \bm{l}_x) \mapsto \textbf{r} := (\bm{n}_r, \bm{l}_r)
\end{equation}
Here the $\bm{n}_r$ are resource nodes and $\bm{l}_r$ are resource links. The graphical depiction is the same as Figure~\ref{disco} except that instead of getting a puffed up graph where the nodes are candidate sets, a standard graph is returned where each node is the chosen resource to underpin an experiment element.

One of the principle features Merge aims to provide is interactive realization.
What this means from a design standpoint is that the algorithms that implement realization need to be fast and reliable.
One could imagine an architecture for a system that accomplishes the same things as Merge, but is based on a fully distributed design.
In this case the implementation of the core services would require fully distributed locks.
In particular, every realization request would require a mutual exclusion envelope that includes at least two global snapshots, one for the state sufficient to run the embedding algorithm and subsequently another one for the reservation of the selected resources pending a successful embedding computation.
The envelope could be implemented pessimistically with a lock, which goes scale-fail very quickly (for obvious lock the world reasons) with a large resource base.

Alternatively if implemented optimistically, transactional rollback and retry under load (another two snapshots per) adds up very fast.
With cross country round trip times anywhere between 50-200 ms and the large number of round trips required to reach a consistent snapshot, the fully distributed approach will be neither fast nor reliable.
A Paxos or Raft-like \cite{paxos,raft} protocol supporting dynamic membership would have to be implemented across the entire network.
Alternatively, limiting the dispersion of critical state to a scale out environment with high-performance databases and reliable fast networks specifically designed to take on this sort of concurrent workload at scale seems a much better choice.

Owing to the scalable representation model on which Merge is based, the realization engine is also scalable in the sense that it naturally evolves along with experiments and the resource base.
The realization and discovery engines operate over XIR representations.
The one assumption XIR makes about the models it represents is that the structure is that of a network. 
XIR has the semantics of a network (in the connected elements sense not the data network sense) cooked into the representation.
Every node and link in an XIR network has a set of properties associated with it.
These properties manifest themselves in one of two ways depending on what is being represented.
If an experiment element is being represented, these properties are fuzzy in that they are represented by constraints.
If an resource element is being represented the properties are concrete.

As a simple example consider a model of an IoT network that may be part of an experiment as shown in Listing \ref{iot-code}, showcasing how properties are able to represented as constraints in XIR.
This model uses the Python language bindings for XIR.
Looking at the interconnect between the \texttt{breaker} and \texttt{xbeehub} nodes we see that the experimenter requires that the communications stack be \texttt{zigbee}, the bandwidth is no greater than \texttt{100 kbps} and the loss rate on the link is greater than \texttt{5\%}.
Furthermore, XIR allows experimenters to specify requirements through key-values (such as operating system, or memory).

% minted pkg: ftp://ftp.dante.de/tex-archive/macros/latex/contrib/minted/minted.pdf
\begin{code}
\begin{minted}
[
frame=none,
framesep=2mm,
baselinestretch=1.2,
fontsize=\footnotesize,
xleftmargin=1cm,
linenos
]{python}
breaker = topo.node({
    'name': 'breaker',
    'image': select('riot'),
    'memory': { 'capacity': gt(xir.mB(256)) },
})
xbeehub = topo.node({
    'name': 'xbeehub',
    'image': choice([
        select('debian-9'),
        select('ubuntu-snap')
    ])
})
topo.connect([breaker, xbeehub], {
  'stack': eq('zigbee'),
  'bandwidth': lt(xir.kbps(100)),
  'loss': gt(xir.percent(5))
})
\end{minted}
%LT: my hacks for getting the spacing right for the caption.
\captionsetup[listing]{position=below,skip=-10pt, justification=centering}
\vspace{18pt}
\captionof{listing}{Describing a topology in Python XIR}
\label{iot-code}
\end{code}

% When a resource elements are expressed, their properties are simply values.
\vspace{3mm}
The job of the realization and discovery engines is one of matching.
They understand a standard set of constraint operators and how to match the data types bound by those operators to concrete values in resource specifications.
Like every other core component, realization and discovery are tied to well defined interfaces.
This means that the underlying implementation can be changed easily or there may be multiple implementations active at a time and users can specify which they would prefer.
Currently, we have two implementations of the realization engine.
One is a simple greedy heuristic like the one presented as the base model in \cite{vni}.
The other is based on an off-the-shelf general satisfiability (SAT) solver, PicoSAT \cite{picosat}.

% There are many choices in representing the realization problem as an instance of satisfiability (SAT).
%In the simplest, each potential match of a requested node to a suitable resource is represented as a binary variable, and logical clauses are added to ensure that exactly one such variable will be true in a solution.
%Link constraints are examined to introduce further pairwise exclusivity constraints between resource mappings.
%The resulting SAT instance can typically be solved efficiently by an off-the-shelf solver such as PicoSAT \cite{picosat}.
%LT: Jim wrote the above, not sure how best make it flow.


%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%         Materialization 
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Materialization}
\label{materialize}

Materialization is the process by which Merge transitions an experiment from the realized to materialized state.
When an experiment has been realized, it means that the resources necessary to instantiate it have been computed and allocated.
Materialization is the process of provisioning the resources selected in the realization phase according to the data specified in an experiment model.
Provisioning a resource according to data in an experiment model can mean a wide variety of things.
Consider two very different examples: an experiment specifies a node has a particular operating system, and an experiment specifies that an industrial control device is configured with a referenced IEC-61131 program.
The materialization engine accommodates both of these use cases, but knows nothing of operating systems or IEC-61131.
In fact the materialization has very little to do with provisioning, all of the real work of provisioning is delegated to drivers, which are described later in Section~\ref{site}.
The primary goal of the materialization engine is to orchestrate provisioning across a distributed network of resources.

To carry out provisioning over a distributed network, we have modeled the materialization engine after the Kubernetes \cite{kube} state convergence model, which solves a similar problem.
When a materialization for an experiment is started, every component of that experiment gets an entry in a data structure called a \emph{stateboard}.
%The stateboard is kept in the transient data store described earlier.
The stateboard is a 2-level (\texttt{experiment-id}, \texttt{resource-id}) lookup table that maps an unique identifiers for an experiment resource to the associated materialization state.
%We need a 2-level lookup because the first lookup is using the experiment's unique identifier, the second lookup is using the resource's unique identifier from within the given experiment.
%The two level aspect comes from the fact that each experiment has a unique identifier and each element within that experiment also has a unique identifier.
% The materialization state is defined as the following data structure.
% LT: unclear to me why the reader cares about 2-level look ups?  Is there an impact?  Is it good, is it bad?

%\begin{minted}{go}
%struct MzState {
%  current, target string
%  version         int
%}
%\end{minted}

Each entry in the stateboard starts at the \texttt{zero} state, with a target state of \texttt{configured}.
The state transitions in between will be discussed in Section~\ref{driver}. It is the materialization engines responsibility to drive each elements state from \texttt{current} to \texttt{target}.
It accomplishes this through a set of agents that are continually monitoring the stateboard.
When an agent finds an entry where the current state is not equal to the target state, it tries to acquire a lease that gives it the right to claim responsibility for driving the \texttt{current} state to the \texttt{target} state.
Architecturally, claiming a lease is required to be an atomic transaction, and the state of each entry must be guarded by a claim.
This allows the agents to scale, and is sufficiently general to allow for swapping out the underlying data store technology if desired.
%In the referenced designs we use etcd \cite{etcd} for this purpose.
% LT: commented out because currently the reference implementation is absent

When it comes to imparting a provisioning action on a resource, the materialization agents work via delegation.
They collect the information from the experiment database that is required to provision a particular resource and then pass that information on to the driver responsible for performing the provisioning.
The materialization agent does not know which driver to contact.
However, it does know what resource provider's site a resource is associated with, and how to look up the model for that site in the site's data store.
Each site model includes a fully qualified domain name that the site commander can be contacted at.
The commander acts as a proxy between the materialization agents running in the core and the various resource drivers running within sites.
Thus the job of the materialization agent is one of ensuring state convergence by delegation.
%This obviously presumes a common state machine model that exists between the materialization agents and the drivers, which is covered in Section \ref{site}.
%We will cover the state machine model in the drivers section.
% can the 2-level lookup be used to go from site -> resource -> experiment?

%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%
%%%
%%%        Commissioning 
%%%
%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%%

\subsection{Commissioning}

Commissioning is the process by which resources are added to and removed from a Merge managed ecosystem.
The unit of commissioning and decommissioning is an XIR network.
This includes everything from a single node network to a complex interconnected fragment of a resource provider's switching mesh.
Figure~\ref{commission} shows the two basic modes of commissioning and decommissioning, \emph{simple} and \emph{fragmented}.

%RY: yes readability issues - ....later
\begin{figure}[ht]
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=.95\columnwidth]{img/commission-simple}
    \caption{Commissioning - Simple Case}
    \label{commission-simple}
\end{subfigure} %
\begin{subfigure}{\columnwidth}
  \centering
  \includegraphics[width=.95\columnwidth]{img/commission}
  \caption{Commissioning - Fragmented Case}
  \label{commission-fragmented}
\end{subfigure} %
\caption{Commissioning simple and complex XIR networks}
\label{commission}
\end{figure}

In the simple case, resources can be commissioned and decommissioned atomically. Consider the example of Figure~\ref{commission-simple}.
In this case the initial commissioning starts out empty.
Then a network is added in a single commissioning request, later the operator of that site decides to take a few nodes away from Merge's control.
This decommission request involves four nodes.
The resulting network is shown as the final diagram on the far right of Figure~\ref{commission-simple}.
This case is considered simple because there are no resources that are impacted besides the ones being commissioned or decommissioned.

In Figure~\ref{commission-fragmented}, we consider the slightly more complex case of fragmented commissioning.
In this example we start with an already commissioned set of resources.
Then the red-highlighted nodes are removed from the commissioning for external use by the site administrator.
In this case, the nodes are a part of a folded Clos network and the removal of nodes has an impact on other elements in the network model i.e., the external use of these nodes will continue to consume resources throughout the network topology. 
In particular the backplanes of the switching elements highlighted in orange will be reduced, but in a way that is invisible to the Merge resource allocation mechanisms. 
Thus the model must be modified to account for this loss in bandwidth.
%As a concrete example, consider the nodes to be connected to their TOR switches at \texttt{10 gbps} and the TOR swtiches connected to fabrics with a \texttt{160 gbps} trunk and the fabrics connected to spines through \texttt{320 gbps} trunks. The allocation of nodes has subsequent allocations all the way up the topology fabric that must be accounted for. When nodes are decommissioned this accounting cannot be done by Merge, so the intermediary switch models must have their bandwidths reduced accordingly.

In the core, Merge simply understands resource addition and subtraction in a very abstract sense.
It has no intelligence about how network capacity properties propagate across a network topology.
It is the responsibility of site administrators to calculate accurate networks as input to the commissioning and decommissioning APIs.
% LT: missing a transition here, but more importantly, what is the take away from fragmented networks?  That resources cant be pulled if they are intertwined with experiments?

